Review of Video Predictive Understanding: Early Action Recognition and Future Action Prediction

Video predictive understanding encompasses a wide range of efforts that are concerned with the anticipation of the unobserved future from the current as well as historical video observations. Action prediction is a major sub-area of video predictive understanding and is the focus of this review. This sub-area has two major subdivisions: early action recognition and future action prediction. Early action recognition is concerned with recognizing an ongoing action as soon as possible. Future action prediction is concerned with the anticipation of actions that follow those previously observed. In either case, the \textbf{\textit{causal}} relationship between the past, current, and potential future information is the main focus. Various mathematical tools such as Markov Chains, Gaussian Processes, Auto-Regressive modeling, and Bayesian recursive filtering are widely adopted jointly with computer vision techniques for these two tasks. However, these approaches face challenges such as the curse of dimensionality, poor generalization, and constraints from domain-specific knowledge. Recently, structures that rely on deep convolutional neural networks and recurrent neural networks have been extensively proposed for improving the performance of existing vision tasks, in general, and action prediction tasks, in particular. However, they have their own shortcomings, \eg reliance on massive training data and lack of strong theoretical underpinnings. In this survey, we start by introducing the major sub-areas of the broad area of video predictive understanding, which recently have received intensive attention and proven to have practical value. Next, a thorough review of various early action recognition and future action prediction algorithms are provided with suitably organized divisions. Finally, we conclude our discussion with future research directions.

==> BODY/chapter1.tex <==
        % \section{Temporal Sequence modelling}

% Background text...
Video data is one type of time-series data. Even though it differs greatly from other such data (\eg speech, text or stock prices) in spatial dimenstionality (\ie each frame of video is a 2-D matrix) and value distributions (i.e., video normally owns three red, green and blue (RGB) channels with ranges determined by the viewed scene and imaging processes), the temporal dimension of videos exhibits some common attributes with other time series, \eg casual relationships between past and future, periodic correlations and smooth transitions, albeit with occasional discontinuities. From this perspective, much work has focused on applying classical temporal sequential modelling to solve video processing tasks.

In this chapter, we review a few major temporal sequential modelling tools that have shown promising results in applications to video understanding. They are Markov Chains, Hidden Markov Models, Bayesian recursive filtering, Gaussian Processes, Auto-Regresstive Models and finally Recurrent Neural Networks. Significantly, the intuition behind these classic tools is greatly shared by the majority of modern approaches but in a more flexible form, which retrospectively underlines the importance of understanding fundamental ideas.

Along with the introduction of basic ideas, concrete cases studies of those methodologies with attention to video sequence data are provided.  

\section{Markov Chains}

Let a time series be defined as an ordered sequence
%Define a time-series data as an ordered sequence:
\begin{equation}
    y_{1:t} = y_{1}, y_{1}, \ldots, y_{t},
\end{equation} 
where one can consider the \textbf{past} and \textbf{future} in the sequence corresponding to ordered indices such as $(1, 2, \ldots, \mathrm{t})$.

A first-order Markov Chain is a standard approach to modelling series of random variables, subject to the constraint that each state depends only on the previous one
\begin{equation}
    p(y_{t} | y_{t-1}).
\label{eq:markov_chain}
\end{equation}
The probability distribution of state transitions is typically represented in terms of the Markov chain’s transition matrix, which often is a stochastic matrix whose entries in each row must add up to exactly one. For $M$ states in the Markov Chain, the transition matrix would be a $M \times M$ matrix.
%A quick example would be forecasting weather based on today's situation through transition matrices, which will be discussed jointly with Hidden Markov Models (HMMs). 

More generally, the model can be extended to ${N_{th}}$ order such that longer dependency is captured:
\begin{equation}
    p(y_{t} | y_{t-1}, y_{t-2}, y_{t-3}, ..., y_{t-N}).
\end{equation}

From the perspective of graphical probability theory, a Markov chain is a directed graph where each temporal state $y_{t}$ has inward connections from one of more previous states (\eg $y_{t-1}$) and outward connections to one or more future states (\eg $y_{t+1}$), as illustrated in Figure \ref{fig:markov_chain}.
\begin{figure}[ht]
    \centering
    \begin{minipage}{.45\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{Figures/HMMs.pdf}
        \subcaption{(a)}\label{fig:sub-a}
    \end{minipage}
    \begin{minipage}{.45\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{Figures/HMMs_2.pdf}
        \subcaption{(b)}\label{fid:sub-b}
    \end{minipage}
\caption{First- (a) and second-order (b) Markov Chain models.}
\label{fig:markov_chain}
\end{figure}

%Markov Decision Process (MDP) \cite{puterman2014markov}, an extension of Makov Chain, is often used in computer vision. MDP extends the vanilla sequential modelling equation \ref{eq:markov_chain} with two extra components: the action space $(a_1, a_2, \ldots, a_t)$ and reward space $(r_1, r_2, \ldots, r_t)$. The actions represent the policy that would decide the transition among observed states
%\begin{equation}
%    p(y_{t} | y_{t-1}).
%\end{equation}
\pagebreak

\section{Hiddens Markov Models (HMMs)}\label{Sec:Temporal_hmm}
A Markov chain is useful when we need to compute a probability for a sequence of observable events. In many cases, however, the events we are interested in are hidden: We do not observe them directly. For example, we might not normally observe the velocity directly from a walking pedestrian. Rather, we might be given geometric distance and time intervals, and must infer the velocity from the ratio of relative moving distance and aggregated time window. We view the velocity as a hidden state because it is not observed.

Formally, we define a Hidden Markov Chain in terms of a sequence of hidden states as $x_{1:T}$, where $T$ is the sequence length, and another sequence of observed variables as $y_{1:T}$. In particular, we define the hidden variable as the causal factor to observations and assume the Markov property for underlying hidden states:
\begin{equation} 
    p(x_{t} | x_{t-1})
\label{eq:1st_markov}
\end{equation}
and
\begin{equation}
    p(y_{t} | x_{t}) = p(y_{t} | x_{t}, x_{t-1}, ..., x_{1}, y_{t-1}, y_{t-2}, ..., y_{1}).
\end{equation}

The estimated probability for an observation at time $t$, $p(y_{t}|x_{t})$ (given its hidden state $x_{t}$), is called the \textbf{emission probability}, which can be used as the inference result when generating outputs. Again, the dynamics behind the hidden sequence is modeled by transition matrices (often denoted as $A$), which can be either invariant to time (\textbf{Homogenous}) or dependent on time (\textbf{Non-Homogenous}). Finally, since every output and state of a sequence is modeled as a probability, an HMM model can be described as generative modelling on sequences as follows
\begin{equation}
\begin{aligned}
    p(x, y) &= p(x_1, ..., x_t, y_1, ..., y_t) \\
            &= p(x_1)p(y_1 | x_1) \displaystyle\prod_{i=2}^{T} p(y_i | x_i) p(x_i | x_{i-1}),            
\end{aligned}
\end{equation}
where $p(x_1)$ and $p(y_1 | x_1)$ are the starting state and observation that are assumed to be independent. Figure \ref{fig:hmm} provides a brief view of this process.

\begin{figure}[htp]
    \centering
    \resizebox{.65\linewidth}{!}{\includegraphics[width=4cm]{Figures/hmm.pdf}}
    \caption{Probabilistic graph model for temporal Hidden Markov Model.}
    \label{fig:hmm}
\end{figure}

HMMs have been applied to a wide range of video understanding tasks, \eg video-based face, finger-spelling and activity recognition \cite{liu2003video,kim2013fingerspelling,raman2016activity}, tracking \cite{yang2016temporal,ullah2018directed} as well as action segmentation \cite{richard2018neuralnetwork, li2019weakly,richard2017weakly, kuehne2018hybrid}. Though these tasks arise in separate settings, research shares many common procedures in their applications. In general, there are three steps in the process. The universal first step involves feature extraction and selection. 
As examples, efforts have converted videos of faces to sequences of eigenvectors \cite{liu2003video}, represented sequences of human appearance as Histograms of Oriented Gradients (HOG) \cite{dalal2005histograms} and represented human motion sequences in terms of Improved Dense Trajectories (iDTs) \cite{wang2013action} with Fisher Vector (FV) encoding \cite{sanchez2013image}, all prior to HMM training.
%For instance, X. Liu \etal, convert the video face images into a sequence of eigenvectors, M. Yang \etal, advocate to use \textit{histogram of oriented gradients} (HOG) feature as an effective representation for human appearance and A. Richard \etal, adopt \textit{improved dense trajectory} (iDT) \cite{wang2013action} feature encoded with \textit{Fisher Vector} (FV) \cite{sanchez2013image} before perform the training of HMM.

The second step is to define a generative model that induces a training process for model parameters. There are three parts of an HMM that need parameter learning from training data: 

\begin{enumerate}
  \item The starting state probability $p(x_1)$; 
  \item The transition probability $A = p(x_i | x_{i-1})$;
  \item The emission probability $p(y_i | x_i)$ that maps hidden states to observations.
\end{enumerate}

The standard choice for initializing the former two components is the uniform distribution, while the standard choice for the third is the Gaussian Mixture Model (GMM) (\eg \cite{yang2016temporal}). Typically, these parameters are jointly learned through the Expectation Maximization (Baum-Welch) algorithm \cite{dempster1977maximum} with an objective to maximize a posterior (MAP).
\begin{figure}[htp]
    \centering
    \resizebox{.55\linewidth}{!}{\includegraphics[width=4cm]{Figures/neural_viterbi.png}}
    \caption{\textcolor{red}{Temporal HMM decoding for action segmentations}, with HMMs implmented as learnable neural networks \cite{richard2018neuralnetwork}.
    The class label for the $i_{th}$ segment is denoted as $c_i$ and the segment length denoted as $l_i$. The input video is forwarded through the network and the Viterbi decoding is run on the output probabilities. The frame labels generated by the Viterbi algorithm are then used to compute a framewise cross-entropy loss on which the network gradient is computed. Figure reproduced from \cite{richard2018neuralnetwork}.}
    \label{fig:hmm_decoding}
\end{figure}

\begin{figure}[]
    \begin{minipage}{\textwidth}
        \centering
        \resizebox{.625\linewidth}{!}{\includegraphics{Figures/hog_hmm.pdf}}
        \caption{Example of using HMMs for video human tracking. Appearance features (upper-row) for each detected pedestrian are extracted via Histogram of Oriented Gradient (HOG) and used for building an observation density shown as sphere nodes in lower graph. 
        The number on nodes $\{1, 2, 3, 4\}$ and blue arrow denote the temporal evolution of observations.
        The state transition is shown as edges between nodes as solid lines. An HMM is built for each pedestrian in the training set and tested on each detected pedestrians during testing. Figure reproduced from \cite{yang2016temporal}.}
    \label{fig:hmm_tracking}
    \end{minipage}
\end{figure}

The third step in applying an HMM to a (video understanding) problem is inferring the end-goal from the emission probability function; namely, \textbf{what is the most likely sequence label given an observed test sequence?} Since HMMs are generative models, instead of discriminative ones, there are two ways to achieve classifications. The first approach assumes the sequential hidden states can represent class labels and thereby the best-fit states would be taken as classification results (typically dubbed HMM decoding) via the Viterbi algorithm \cite{forney1973viterbi} according to:
\begin{align*}
    y* &= \operatorname*{argmax}_{y \in {y_1, \ldots, y_T}} p(x_1, ..., x_t, y_1, ..., y_T) \\
       &= \operatorname*{argmax}_{y \in {y_1, \ldots, y_T}} p(y_1)p(x_1 | y_1) \displaystyle\prod_{i=2}^{T} p(x_i | y_i) p(y_i | y_{i-1}).
\label{eq:hmm_decoding}
\end{align*}
However, this approach is not easily applicable to datasets that contain a large number of classes, where the number of states increase linearly in proportion to the size of categories. As a remedy, the second approach is through training HMMs for each class cateogory in the datasets of interest. In the classification phase, given a target video, we would first make an observation sequence and feed it into every HMM. By evaluating the probability for each HMM, the target video is assigned into a class based on the highest HMM probability.

%For recognition tasks, each HMM model learned on each class of training set would produce likelihood scores by fitting test data into the learned emission probability function and pick the maximum likelihood model. Typically, the best-among-N is taken as the class index. Temporal action detection is similar to recognition, except that at each time step the class of the performed action is to be preserved without aggregation. Tracking can be similarly framed as discrimination of each detected pedestrian with pre-trained HMM models.
Both classification methods have been applied to computer vision tasks. As an example for the HMM decoding approach, some work proposed a neural-network implemented Viterbi decoding HMM to infer the segment-wise action label \cite{richard2018neuralnetwork}; see Figure \ref{fig:hmm_decoding}. Similar work includes \cite{kuehne2018hybrid, li2020set, koller2017re}. As for the second approach, an effort has proposed to incorporate HMMs with appearance features (HOG) for pedestrians tracking \cite{yang2016temporal}; see Figure \ref{fig:hmm_tracking}. Each newly detected pedestrian is tested with all pre-trained HMMs to associate with an existing pedestrian template. 

%A. Richard \etal \cite{richard2018neuralnetwork} proposed a neural-network implemented viterbi decoding HMM to infer the segment-wise action label (see Figure \ref{fig:hmm_face} segment class denoted as $c_i$ and segment length denoted as $l_i$).
%As an example for the second approach, M. Yang \etal \cite{yang2016temporal} proposed to incorporate HMMs with appearance features (HOG) for pedestrians tracking, as shown in Figure \ref{fig:hmm_tracking}. Each newly detected pedestrian would be tested with all pre-trained HMMs to associate with existing pedestrian template. 

Other related work explores the possibility of extending the expressiveness of HMMs. One direction is to enrich the hidden states by stacking them in hierarchical fashion \cite{raman2016activity}. Another is to relax the assumption on prior distributions for learning parameters (the initial distribution, the transition matrix and the emission matrix). A currently trending approach to relaxing these assumptions is grounding the HMM as a learnable Recurrent Network Network (RNN) \cite{richard2018neuralnetwork, richard2017weakly, li2019weakly}.

%Abovementioned operations are necessary to properly execute HMMs which, on the other hand, reveals several limitations: \textbf{1.} expensive and slow to run optimization algorithms (EM algorithm run time increases dramatically with the number of hidden states); \textbf{2.} difficult to extend the dependency from lower order to higher; \textbf{3.} unable to perform online inference due to the prerequisite for fixed temporal data length during training.

Finally, it is important to note that the necessary operations to yield a classic HMM reveal several limitations. First, they can be expensive and slow to run their optimization algorithms (e.g., model run time increases dramatically with the number of hidden states). Second, extensions to high-order models can be very complicated. Third, the ability to do inference on variable length input data requires a time-invariant transition matrix, $A$, which is often less expressive than time-variant ones.

%Third, online inference can be difficult to achieve because of the prerequisite of fixed temporal length during training \cite{}.

\section{Bayesian Filtering}
The problem of temporal \textit{filtering} is an operation that involves the extraction of information about a quantity of interest at time $t$ by using data measured up to and including $t$ \cite{chen2003bayesian}. (Here, we ignore the possibility of noncausal filters). We define a generic form of the filtering problem from the perspective of the dynamic state-space system over a sequence of state variables, $(x_1, \ldots, x_T)$, and time-measured observations, $(y_1, \ldots, y_T)$:
\begin{equation}
\centering    
\begin{aligned}
    &x_{t+1} = f(x_t, q_t) \\
    &y_{t} = h(x_{t}, r_t).
\label{eq:genric_filtering}
\end{aligned}
\end{equation}
In the above formulation, $x_t$ represents the state vector at a given step, while $y_t$ stands for its observation; $q_t$ and $r_t$ represent the process noise and measurement noise at time $t$, respectively; $f$ and $h$ are functions that model physical relationships between adjacent states and measurements, respectively. More specifically, the state function, $f$, is responsible for transitioning state vectors forward in time, which characterises the transition probability, $p(x_{t+1} | x_t)$, and the measurement equation, $h$, for mapping the states to an estimated observation vector, which captures the measurement probability, $p(y_{t} | x_{t})$. 

This formula is widely adopted in modelling many real-world physical systems (\eg estimating airplane locations or robot trajectories) and the quantity of interest that researchers attend to hereby is the state vector $x_t$ (\eg velocity, gravity force or air resistance). In other words, the \textbf{objective} of filtering is to estimate the posterior density $p(x_t | y_{1:t})$ at any given step.

Bayes' theorem builds the fundamental formulation for conditional probability $p(y|x)$ with its inverse conditional probability $p(x|y)$ and the marginal probabilities $p(y)$ and $p(x)$ as follows. This formulation naturally fits the purpose of filtering \cite{ho1964bayesian}, especially when states and observations are treated as random variables subject to certain distributions. The theorem is given as
\begin{equation}
    p(x | y) = \frac{p(y|x) p(x)}{p(y)},
\label{eq:bayes_rule}
\end{equation}
where $p(x)$ represents the \textbf{\textit{prior}} knowledge we have about the states, $p(y|x)$ is the \textbf{\textit{likelihood}} probability, while the denominator, $p(y)$, stands for the probability of observing $y$ happening, which usually gets taken as a constant value due to its independence from the targeted state variables. Therefore, the central idea of Bayesian inference is to use priors and likelihood knowledge, quantitatively and qualitatively, to infer the conditional probability, given tractable observations, which corresponds to the goal of filtering. However, vanilla Bayes theorem is not directly applicable to sequential data, as there is no linkage between data in time.


Formally, Bayesian filtering is defined as a combination of the Markov property and Bayes rule with two major assumptions \cite{chen2003bayesian}: \textbf{1.} The hidden states follow a first-order Markov process $p(x_t | x_{1:t-1}) = p(x_t | x_{t-1})$; \textbf{2.} The real measurements, $y_t$, are independent of the given states. The conditional probability density function of $p(x_t | y_t)$ thus can be described as:
\begin{equation}
\centering    
\begin{aligned}
p(x_t|y_t) &= \frac{p(y_t | x_t) p(x_t)}{p(y_t)} \\
           &= \frac{p(y_t, y_{t-1} | x_t) p(x_t)}{p(y_t, y_{t-1})} \\
           &= \frac{p(y_t|y_{t-1}, x_t)p(y_{t-1} | x_t) p(x_t)}{p(y_t | y_{t-1}) p(y_{t-1})} \\
           &= \frac{p(y_t|y_{t-1}, x_t)p(x_t | y_{t-1}) p(y_{t-1}) p(x_t)}{p(y_t | y_{t-1}) p(y_{t-1}) p(x_t)} \\
           &= \frac{p(y_t | x_t) p(x_t | y_{t-1})}{p(y_t | y_{t-1})}.
\label{eq:bayes_filtering}
\end{aligned}
\end{equation}
Under these assumptions, the prior becomes
\begin{equation}
p(x_t | y_{t-1}) = \itt p(x_t | x_{t-1}) p(x_{t-1} | y_{t-1}) dx_{t-1},
\end{equation}
which represents the newly propagated states only from the very last step posterior, $p(x_{t-1} | y_{t-1})$, and the model dynamic, $p(x_t | x_{t-1})$. The likelihood, $p(y_t | x_t)$, and evidence, $p(y_t | y_{t-1})$, serve the same role as before but are self-contained at given time step $t$, without depending on any remote historical states or observations (\eg $t-2$). 
%The graphical model is depicted as Figure \ref{fig:bayesianFilter}. 
The graphical representation of Bayesian filtering is identical to the one given for HMMs in Figure \ref{fig:hmm}.
\iffalse
\begin{figure}[htp]
    \centering
    \resizebox{.5\linewidth}{!}{\includegraphics[width=4cm]{Figures/bayesian_filtering.pdf}}
    \caption{Bayesian filter in graphical presentation behaves in an analogous manner to a first-order hidden Markov model.}
    \label{fig:bayesianFilter}
\end{figure}
\fi

It is worth noticing that the conditional modelling property of Bayesian filtering makes it easier to perform than the Hidden Markov Model, which aims at modelling the joint probability of the entire sequence data pair (\ie observation $y_{i}$ and hidden states $x_{i}$). For every new incoming state and observation, HMMs need to re-run the whole sequence, while Bayesian filtering can do inference conditioned on only the last state.

To this point, the theoretical formulation of Bayesian filtering has been soundly built, though it is still vague on how to implement it with a tractable realization (\ie how to decide the distribution of likelihood and prior). In the next two sections, we present the celebrated Kalman filter and particle filter as concrete examples that realize Bayesian filtering in practice.

\subsection{Kalman Filtering}
Kalman filtering is one convenient instantiation of Bayesian filtering \cite{chen2003bayesian}. It merges the essence of recursive probability estimation with linear differential systems, through assuming \textbf{Linear–Quadratic} dynamics for state variables and \textbf{Gaussian} uncertainty for both the process and measurement noise. Taken together, these assumptions are known as LQG. Consider the same sequence of state-space data from previous section, $(x_1, ..., x_T)$ and $(y_1, ..., y_T)$, the generic filtering equation \ref{eq:genric_filtering} under the LQG assumptions can be re-expressed in a simpler version as:
\begin{equation}
x_{t+1} = F x_t + q_t
\label{eq:kf_pred_1}
\end{equation}
and
\begin{equation}
y_{t} = H x_t + r_t,
\label{eq:kf_pred_2}
\end{equation}
where $F$ is the transition matrix, $H$ is the measurement matrix, $q_t$ and $r_t$ are white Gaussian noise at time step $t$. These two steps are named the \textbf{prediction} step in Kalman filtering, which jointly operationalize the prior transition step, $p(x_t | y_{t-1})$, in Bayesian filtering.

The second step of Kalman filtering is given according to
\begin{equation}
\centering
\begin{aligned}
    &P_{t|t-1} = FP_{t-1}F^{T} + q_t \\
    &K_t = P_{t|t-1}H^{T} (HP_{t|t-1}H^{T} + r_t)^{-1} \\
    &x_t^{MAP} = \hat{x}_{t|t-1} + K_t (y_t - H\hat{x}_{t|t-1}) \\
    &P_t = P_{t|t-1} - K_tHP_{t|t-1},
\end{aligned}
\label{eq:kalman_update}
\end{equation}
where $K_t$ is called Kalman Gain, $P_t$ is the state error covariance matrix, $\hat{x}_{t|t-1}$ is the prior state estimation given observations till $y_{t-1}$ and $x_t^{MAP}$ is the Maximum A Posteriori (MAP) estimate of $x_t$. 
%The detailed deduction of above equations can be found in appendix \ref{appendix:kalman}.
These equations support the posterior estimation from the priors and the likelihood. In practice, they are named the \textbf{update} step since they assimilate the up-till-now incoming observations and inversely correct the predicted states. A detailed derivation of the Kalman filtering equations, (2.13),  from the point of view of Bayesian filtering is provided in Appendix \ref{appendix:kalman}.
The Kalman Gain,
$K_{t}$ , is derived from the ratio of the state uncertainty, $P$, and the measurement noise, $r_{t}$. It balances the prior state estimation, $\hat{x}_{t|t-1}$, and the measurement error, $y_t - H\hat{x}_{t|t-1}$. An accurate system should reduce the $K_t$ term since the prior prediction should be accurate enough to represent the real states.

Besides the Kalman Gain, another equally critical factor is the error covariance, $P_t$, which in nature reflects the covariance of the state vectors, yet numerically focuses on the state residual errors (here assuming the state-error vector is a random variable). 
%Therefore, in equation \ref{eq:prior}, the deduction of the state covariance yields $Cov(x_t | y_{t-1}) =  Cov(e_t|e_{t-1})$.
The predicted state covariance relies on the physical model matrix, $F$, and the process noise, $q$. One step of Kalman filtering is depicted in Figure \ref{fig:kalmanFilter}.
\iffalse
As indicated by Equation \ref{eq:error_prop}, the prediction of the state covariance relies on the physical model matrix, $F$, and the process noise, $q$. For any transition matrix that has numeric elements that are larger than 1 (\ie $|F| > 1$), the state covariance would be amplified. From equation \ref{eq:error_update}, the error covariance will be udpated by re-assigning the prior prediction $P_{t|t-1}$ with the ratio $(I - K_t H) \in (0, 1)$ that depends on the Kalman Gain $K_t$. One iterating step, $t-1$ to $t$, of Kalman filtering is depicted in Figure \ref{fig:kalmanFilter}.
\fi

The most noticable merit of Kalman filtering is its \textbf{optimality}. Given a linear dynamic system model and known Gaussian distributions for noise, the estimated state is guaranteed to match the real system, since the MAP estimation on a linear function can lead to a global optimum.

The most well-known disadvantage of Kalman filtering is its limitation to only \textbf{uni-modal} modelling. Under LQG assumptions, the implementation of the desired posterior is always a \textbf{single} Gaussian parameterized with its moments (\ie mean and covariance). When the target measurement behaves like a mixture of Gaussian distributions that contains more than one modality, the Kalman filter can only follow one mode. 

Another critical flaw of the Kalman filter is the \textbf{Linear} assumption. Though simple and efficient, many higher level vision tasks are better modeled by nonlinear state transitions, in which case the Kalman filter could only provide sub-optimal solutions.
\begin{figure}[htp]
   \centering
    \resizebox{.7\linewidth}{!}{\includegraphics[width=4cm]{Figures/Kalman.png}}
    \caption{Depicting the Kalman filtering process. A Gaussian shape distribution is propagated by iterating steps at each time frame. However, only one Gaussian blob can be processed at a time. Figure reproduced from \cite{wiki:kalman}.}
    \label{fig:kalmanFilter}
\end{figure}

More generally, not all physical rules can be modeled as linear systems. Thus, the \textbf{Extended} Kalman filter (EKF) and \textbf{Unscented} Kalman filter (UKF) \cite{julier1995new} have been proposed to enable more flexible estimation on nonlinear processes. The former admits nonlinear state transition/measurement functions, $f$ and $h$, to replace the previous matrices, $F$ and $H$, so that the Eq. \ref{eq:kf_pred_1} and \ref{eq:kf_pred_2} become
\begin{equation}
    x_{t+1} = f(x_{t})
\label{eq:nonlinear_k}
\end{equation}
and
\begin{equation}
    y_{t} = h(x_{t}),
\end{equation}
respectively.

The \textbf{update} step is the same as Eq. \ref{eq:kalman_update}, except that the matrices used are derived from the \textbf{Jacobian} matrices of $f$ and $h$, namely $F = \frac{\partial f}{\partial x}$ and $H = \frac{\partial h}{\partial x}$ (first-order Taylor expansion), which represents a linear approximation to nonlinear functions and therefore can not guarantee optimal estimation. The UKF further relieves the \textbf{update} step from the linear constraint by resorting to a sampling approach, but ends up being expensive on computational resources.

\textbf{Applications:} The Kalman filter has been applied widely in fields like computer vision, robotics and navigation systems. Concrete examples include the Global Positioning System (GPS), Unmanned Aerial Vehicles (UAV) and tracking of human trajectories or motions assisted with technologies from signal processing, sensor information and computer vision. Precedents found success when coupling Kalman filtering with physical law based motion models, \eg velocity, acceleration, moving angle, airflow resistance and gravity. In the instance of video-stream vehicle tracking, people found it useful to use the EKF with vehicle's positions, speeds and turning angles as state variables to track the observed coordinates \cite{guerrero2013vehicle}. The main theme is finding an applicable physical model for the state transition.
\iffalse
As a simple example, 
consider tracking objects in a 2D X-Y plane. We can build a simple Kalman filtering system to achieve this goal. First, the state vector $\mathbf{x}$ is explicitly defined as
%exmple from: https://github.com/balzer82/Kalman/blob/master/Kalman-Filter-CA-2.ipynb;
\begin{equation}
\centering
\mathbf{x} =
\begin{bmatrix}
    x\\
    y\\
    v_x\\
    v_y\\
    a_x\\
    a_y\\
\end{bmatrix},
\end{equation}
where $x,y$ are coondinates, $v_x, v_y$ are velocities and $a_x, a_y$ are accelerations. Following the physical motion formula $y = x + \Delta t v + \frac{1}{2} \Delta t^2 a; v = v + \Delta t a$, the transition between states can be defined as (assuming constant acceleration):
\begin{equation*}
\centering
    \mathbf{x}_{t+1} = 
    \begin{bmatrix}
        1& 0& \Delta t & 0 & \frac{1}{2}\Delta t^2& 0 \\
        0& 1& 0& \Delta t& 0& \frac{1}{2} \Delta t^2 \\
        0& 0& 1& 0& \Delta t& 0 \\
        0& 0& 0& 1& 0& \Delta t \\
        0& 0& 0& 0& 1& 0 \\
        0& 0& 0& 0& 0& 1
    \end{bmatrix}
    \mathbf{x}_t
\end{equation*}

The measurement, $\mathbf{y}_t$, namely the observed positions, can be expressed from the measurement matrix as
\begin{equation*}
\centering
    \mathbf{y}_t = 
    \begin{bmatrix}
    1 & 0 & 0 & 0 & 0 & 0 \\
    0 & 1 & 0 & 0 & 0 & 0
    \end{bmatrix}
    \mathbf{x}_t + \mathbf{r}_t
\end{equation*}
where $r_t$ is the measurement noise $r_t \sim\ N(0, R)$. The state error covariance $P_t$ is
\begin{equation*}
\centering
    \mathbf{P}_{t+1} = F\mathbf{P}_{t}F^{T} + \mathbf{q}_t = F
    \begin{bmatrix}
        cov_{x,x}& cov_{x,y}& 0 & 0 & 0 & 0 \\
        cov_{y,x}& cov_{y,y}& 0& 0& 0& 0 \\
        0& 0& 0& 0& 0& 0 \\
        0& 0& 0& 0& 0& 0 \\
        0& 0& 0& 0& 0& 0 \\
        0& 0& 0& 0& 0& 0
    \end{bmatrix}
    F^{T} + \mathbf{q}_t
\end{equation*}
where $\mathbf{q}_t$ is the process noise $\mathbf{q}_t \sim\ N(0, Q)$ and similar for $\mathbf{r}_t$.

The noise parameters, $R$ and $Q$, are manually defined beforehand to mimic the real environment. The very initial error covariance $P_1$ also needs to be specified to reflect the initial uncertainty,
but it will eventually converge to a steady value as the process goes on. Figure \ref{fig:KF_example_ball} plots the development of prediction, update and noise measurement of 2D coordinates along time.
\begin{figure}[htp]
   \centering
    \resizebox{.7\linewidth}{!}{\includegraphics[width=4cm]{Figures/Kalman-Filter-CA-Ball-StateEstimated.png}}
    \caption{Kalman filtering example for tracking 2D plane coordinate measurements which follow linear velocity-acceleration motion function.}
    \label{fig:KF_example_ball}
\end{figure}
\begin{figure}[htp]
   \centering
    \resizebox{.7\linewidth}{!}{\includegraphics[width=4cm]{Figures/Kalman-Filter-CA-Ball-KalmanGain.png}}
    \caption{Kalman Gain, $K_t \in (0, 1)$, changing plot. The lower, the more the measurement fullfill the prediction.}
    \label{fig:KF_example_ball}
\end{figure}
\fi
\iffalse
\begin{figure}[ht]
    \centering
    \begin{minipage}{.45\textwidth}
    \includegraphics[width=1.25\textwidth, height=4cm]{Figures/kalman_vehicle.PNG}
    \end{minipage}
    \begin{minipage}{.45\textwidth}
    \begin{flushright}
    \includegraphics[width=.6\textwidth, height=4cm]{Figures/kalman_motion.png}
    \end{flushright}
    \end{minipage}
\caption{Vehicle tracking on street scenes (Left) with assumed motion states equation that involves velocities $v_{x}, v_{y}$, positions $P_{x}, P_{y}$ and directional angle $\phi$ (Right).}
\label{fig:kalman_vehicle}
\end{figure}
\fi
\iffalse
All abovementioned methods (KF, EKF, UKF) rely on pre-defined motion models as transition functions. No matter how complicated, they are not easily adaptale to out-of-domain data and lack the ability to explore unknown motion relations from the data. How to effectively adapt the transition model to our needs remains an open question.
\fi
Reliance on pre-defined motion models across the Kalman filter and its standard variants (EKF, UKF), makes them not easily adaptable to out of domain data and limits their ability to explore uknown motion relations in the data. How to effectively adapt transition modelling remains an open question.

\textbf{Learning Based Extensions}: In recent progress of machine learning, Kalman filtering is frequently revisited. Researchers try forging its core concepts into a learning structure with two general goals: \textbf{1.} Alleviating the rigid transition model and Gaussian noise assumption; \textbf{2.} Overcoming the dimensionality curse and extending the application landscape to new horizons.

As an example of the first consideration, an early effort proposed to substitute the transition function $f$ as well as the two noise terms with Long-Short Term Memory (LSTM \cite{hochreiter1997long}) units \cite{coskun2017long}. They apply the proposed LSTM-KF to regularize a series of video human body keypoint estimations and demonstrate that the merged method performs better than a Kalman filter under hand-crafted motion models (velocity and acceleration) as well as a pure learning LSTM network. Similar work includes \cite{dynamet2019chen}. Figure \ref{fig:lstm_kf} provides an illustration.

\begin{figure}[ht]
    \centering
    \begin{minipage}{.4\textwidth}
    \centering
    \includegraphics[width=1.\textwidth, height=4cm]{Figures/lstm_kf.PNG}
    \subcaption{(a)}
    \end{minipage}
    \begin{minipage}{.4\textwidth}
    \centering
    \begin{flushright}
    \centering
    \includegraphics[width=.57\textwidth]{Figures/lstm_kf_body.png}
    \end{flushright}
    \subcaption{(b)}
    \end{minipage}
\caption{(a) Realization of Kalman filtering with LSTM units. The state transition, $p(\hat{y}_{t} | \hat{y}_{t-1})$, and noise terms, $\mathsf{Q}$ and  $\mathsf{R}$, now are the outputs of three learnable LSTM networks, rather than manually defined priors.
(b) Body key-point generation outcomes from distinct implementations. Proposed LSTM-KF approach (highlighted with red rectangular) produces the best result.
Both (a) and (b) reproduced from \cite{coskun2017long}.
}
\label{fig:lstm_kf}
\end{figure}

Other work takes this path one step further \cite{haarnoja2016backprop}. In that work, it is argued that the classic transition function is a generative estimator in the probability world, which has limited capacity to handle rich sensory observations, \ie high resolution images and videos. Indeed, existing work resorted to preprocessing raw data input, \eg obtaining 2-D positions of pedestrians through detectors, prior to Kalman filtering.
\iffalse
\begin{figure}[htp]
  \centering
\resizebox{.95\linewidth}{!}{\includegraphics[width=4cm]{Figures/backprop_kf.png}}
\caption{Discriminative state estimation model emboddied through forward neural network from \cite{haarnoja2016backprop}. This model inputs high-dimensional observations, such as raw images denoted as $o_{t}$, and produces an intermediate observation $z_{t}$ to interlace with the underlying dynamic state $\mu$, which will be used to produce final observation $y_t$.
Two noise terms ($\mathsf{Q}$ and $\mathsf{R}$) are also learned instead of pre-defined. 
}
\label{fig:backprop_kf}
\end{figure}
\fi
In response, the authors advocated a discriminative model that maps raw high dimensional observations to a low dimensional vector
%(denoted as $\mathbf{z}$) 
as an intermediate observation state, together with a positive-definite covariance matrix
%, $L$, 
for constructing the noise.
%($\mathsf{Q}$ and $\mathsf{R}$) 
%, as shown in Figure \ref{fig:backprop_kf}. 
The projected vector
%$\mathbf{z}$, 
works as the measurement in the \textbf{update} step to capture the underlying dependency between observations and states. However, arguably such an extension still deviates from directly applying Kalman filtering to complex visual tasks, since its down-steam output is still low dimensional geometry information (\eg groundtruth output is either tracking coordinates in $\mathbb{R}^{2}$ or visual odometry in $\mathbb{R}^{3}$ that determines the position and orientation of a vehicle by analyzing the associated camera images).

As to the second consideration, extensions to wider applications and overcoming associated dimensionality issues, recent breakthroughs have led to the use of Kalman filtering in unpredecented fields, such as video action detection \cite{dave2017predictive}, video artifact reduction \cite{lu2018deep}, temporal feature propagation \cite{zhao2019spatiotemporal} and video pixel prediction \cite{guen2020disentangling}. Theses efforts share two common attributes: \textbf{1.} The \textbf{predict-update} functionality is extended to visual and semantic feature spaces; \textbf{2.} Video frame-wise \textbf{residuals} are found complementary to Kalman filtering mechanisms.

%For example, A. Dave \etal \cite{dave2017predictive} firstly propose to incorporate Kalman structure onto video action semantic detection. 
As an example, it has been proposed to incorporate the Kalman structure into action semantics detection \cite{dave2017predictive}.
In that framework, the noise terms ($q_t, r_t$ of Equations \ref{eq:genric_filtering} and \ref{eq:kalman_update}) are ignored (since the task has marginal relation with state uncertainty) and the semantic action activation layer in a deep ConvNet at every time-step is a linear combination of such features from the previous step and a corrective (residual) term distilled from raw image observations. Notably, such high dimensional representation was prohibitive in earlier eras due to lack of computational resources; see Figure \ref{fig:CNN_KF_Detection} for the predictive-corrective component of \cite{dave2017predictive}.

\begin{figure}[htp]
   \centering
    \resizebox{.85\linewidth}{!}{\includegraphics[width=4cm]{Figures/CNN-KF-Detection.pdf}}
    \caption{Proposed predictive-corrective action detection framework that filters two adjacent observations $t \in (1, 2)$ in \cite{dave2017predictive}. ConvNet (denoted as CNN) is used as the key technique to perform state transit between time steps. Previous prediction at each step will be corrected by the next observation and thus the propagation error is not accumulated. Figure reproduced from \cite{dave2017predictive}.}
    \label{fig:CNN_KF_Detection}
\end{figure}

Various efforts have followed this general idea. One such effort thinks of the predicted video pixel residual as the corrective add-on, which shares the same resolution with original images \cite{lu2018deep}. Others choose to predict the temporal residual of the intermediate ConvNet features \cite{guen2020disentangling, zhao2019spatiotemporal}, since the middle layer preserves rich spatial structure information, and update the recovered feature with real measurements. 
%However, there are some subtle distinctions between them, \ie \cite{zhao2019spatiotemporal} uses deep features with resolution (28x28x192), while \cite{guen2020disentangling} uses (7x7x128).

One possible reason why Deep-Kalman proposals can enhance complex video tasks is that advances from machine learning theory help overcome the long-existing struggle to model high dimensional data. Here, the residual term is essential, since large portions of video data contains redundancy with adjacent frames. By modelling the adjacent residual, models are taught to focus on the dynamic part (\ie on-going action movements or walking pedestrians) rather than static ones (\ie backgrounds).

Beyond the abovementioned uses of Deep Kalman filtering in computer vision tasks, such an idea also has been investigated in the traditional machine learning literature. As examples, a hybrid model that combines physical dynamic rules, learning based transition matrices and latent variables was investigated to estimate the trajectory of a noisy chaotic Lorenz Attractor \cite{satorras2019combining}. Another effort approached Kalman filtering with a variational inference backbone \cite{kingma2013auto} and then modeled the change of a patient’s state over time \cite{krishnan2015deep}. Further similar work includes \cite{karl2016deep, rangapuram2018deep}. Again, these efforts relaxed the LQG assumptions of standard Kalman filtering. Parallel work devoted to supporting high dimensional data modelling in Kalman filtering suggested factorizing latent variables into low dimensional data (even scalars) \cite{becker2019recurrent}.  The authors also relied on recurrent neural networks to enable nonlinear dynamics for the state transition.


%Similarly, G. Lu \etal \cite{lu2018deep}, H. Zhao \etal \cite{zhao2019spatiotemporal} and V. Le Guen \etal \cite{guen2020disentangling} all succeed this idea. Lu thinks of the predicted video pixel residual as the corrective add-on, which shares the same resolution with original images (height:448, width:256). Instead, Zhao and Guen focus on predicting the temporal residual of the intermediate ConvNet features (28x28x192 and 7x7x128 respectively), since the middle layer preserves rich spatial structure information, and update the recovered feature with real measurements.
\iffalse
\begin{figure}[ht]
    \centering
    \includegraphics[width=.6\textwidth, height=4cm]{Figures/pred_cor_kf2.PNG}
\label{fig:deep_kf}
\caption{Generic description of deep Kalman approach for high-dimensional visual observation or semantic feature from \cite{dave2017predictive}.}
\end{figure}
\fi

\subsection{Particle Filtering}
In this section we describe another famous Bayesian filter, the particle filter. In constrast to the Kalman filter, the particle filter is non-linear and non-Gaussian but is still under the Markov property. That is to say, the dynamics behind the state variable and the noise distribution can be of almost any form. These great merits come from the Monte-Carlo Sampling idea that uses a set of particles to represent target distributions in a non-parameteric fashion. Thus, the particle filter is categorized as a Markov Chain Monte-Carlo (MCMC) \cite{del1997nonlinear} method or \textit{Sequential Monte-Carlo} (SMC) \cite{liu1998sequential}.

Instead of directly calculating the desired posterior, $p(x_t |y_t)$, by assuming a Gaussian distribution, its density can be empirically represented by a weighted sum of $N_p$ samples drawn from the posterior distribution
\begin{equation}
    p(x_t| y_t) \approx \frac{1}{N_p} \sum_{t=1}^{N_p} \hat{w}_{t}^{i} \delta(x_t - x_t^{(i)}) = \hat{p}(x_t | y_t),
\label{eq:pf_posterior}
\end{equation}
where $x_t^{(i)}$ are sampled data points from $p(x_t | y_t)$, $\hat{w}_t^{i}$ are weights and $\delta(\cdot)$ is the Dirac delta function. However, it is impossible to draw data from the optimal $p(x_t | y_t)$ prior to owning its estimation. An alternative is to find a \textit{proposal distribution} $q(x_t | y_t)$ and draw samples from it to approximate $p(x_t | y_t)$. Apparently, not all approximated samples are valid and therefore we should weight the alternative samples according to
\begin{equation}
    w^{i}_{t} = \frac{p(x_{t}^{i}| y_{1:t})}{q(x_{t}^{i}| y_{1:t})}.
\label{eq:particle_weight}
\end{equation}

In practice, this step could be done through calculating the absolute value of the deviation of the measurement from its expected value with a certain evaluation metric (\ie using Chi-square distributions on $p(x_{t}^{i}| y_{1:t})$ and $q(x_{t}^{i}| y_{1:t})$).
Therefore, for a batch of samples $N_p$ at time $t$, the normalized weight $\hat{w}^{i}_{t}$ for the $i_{th}$ sample point is
\begin{equation}
        \hat{w}^{i}_{t} = \frac{w^{i}_{t}}{\sum^{N_p}_{i=1}w^{i}_{t}}.
\end{equation}

Recalling that Bayes' rule and the first-order Markov chain assumption contribute greatly to the derivation of the Kalman filter, the particle filter also benefits from these two assumptions. More specifically, 
we follow Equation \ref{eq:bayes_filtering} and further set $q(x_t | x_{t-1}, y_{1:t}) = q(x_t | x_{t-1}, y_{t})$.
Then, Equation \ref{eq:particle_weight} can be rewritten as
\begin{equation}
    \begin{aligned}
       w^{i}_{t} &\sim\ \frac{
           p(y_t | x_t)p(x_t | x_{t-1})
       }{
           q(x_t | x_{t-1}, y_{1:n})
       } \\
       &= \frac{
           p(y_t | x_t)p(x_t | x_{t-1})
       }{
            q(x_t | x_{t-1}, y_{t})
       }.
    \end{aligned}
\end{equation}

The most common choice for the proposal distribution is the prior probability $q(x_t | x_{t-1}, y_{t}) =p(x_t | x_{t-1})$, thus the weights can be simplified as $w^{i}_{t} = p(y_t | x_t^{i})$. Having obtained both the samples and their weights, the posterior can be easily calculated using Equation \ref{eq:pf_posterior}.
In general, the particle filter operates in the following workflow:
\begin{itemize}
    \item Generate data samples from prior probability.
    \item Assign weights to samples that are valued from observations.
    \item Approximate the posterior with weighted samples.
\end{itemize}

\begin{figure}[ht]
    \centering
    \includegraphics[width=.6\textwidth]{Figures/mc.png}
\caption{Illustration of density representation through particles. Purple circles stand for particles. Larger size of circle means denser (larger quantity) particle clustering and therefore higher the density value, $p(x)$. Figure reproduced from \cite{particle}.} 
\label{fig:particle_density}
\end{figure}
            
The particle filter has both pros and cons. On the pro side, the Monte-Carlo based inference empowers the particle filter supporting \textbf{multi-modality}. In the previous literature, each state variable equals to an uni-modal Gaussian distribution and it is unfeasible to expand them to multivariate. On the contrary, the particle filter enables modelling any-form of distribution through particles (as shown in Figure \ref{fig:particle_density}). Problems that demand multiple outcomes, such as robotic localization and multi-target tracking, are then feasible, see Figure \ref{fig:pf_poor}(b).

On the con side, since sampling based methods rely on valid particles to obtain decent distributions, the first evident disadvantage of the particle filter is the possible need to select a large amount of particles, which can be expensive and non-real time in practice. As shown in Figure \ref{fig:pf_poor}(a), the number of particles plays an important role in adequately matching the target distribution.
\begin{figure}[ht]
    \centering     
    \begin{minipage}{.45\textwidth}
    \centering
    \includegraphics[width=1.\textwidth]{Figures/Histogram-Plots-of-Differently-Sized-Monte-Carlo-Samples-from-the-Target-Function.png}
    \subcaption{(a)}
    \end{minipage}
    \begin{minipage}{.425\textwidth}
    \centering
    \begin{flushright}
    \includegraphics[width=1.\textwidth]{Figures/Screen Shot 2020-09-26 at 2.13.55 AM.png}
    \end{flushright}
    \subcaption{(b)}
    \end{minipage}
\caption{(a) Illustration of the sensitivity of Monte Carlo approaches in terms of the number of samples. Insufficient amount of samples can lead to misinformed estimation.
(b) Example of using the particle filter for robot localization from \cite{fox1999monte}. Red dots represent particle samples that can scatter around multiple possible locations on the floor plan; Green dot is the robot agent that can attend to all possible locations covered by particles (blue lines), which differs from the Kalman filter. Subfigure (b) reproduced from \cite{nummiaro2002color}.}
\label{fig:pf_poor}
\end{figure}
However, owning enough particles can not always guarantee optimality. When there are a few particles dominating the probability weights, while the majority of other particles are near-zero weight, the resulting approximation suffers the same issue as above. This issue is referred to as \textbf{sample degeneracy}. The typical remedy is to remove dead particles, perform resampling and assign them uniform weight. This resetting process is dubbed Sequence Importance Resampling (SIR), which sometimes can lead to another serious problem named \textbf{sample impoverishment}. In the impoverishment issue, resampled particles fail to cover multiple modes or different spatial regions because dominant particles can not cover the whole distribution landscape. Resampling from deficient yet dominating particles leads to equally unsatisfying outcomes.

In spite of these disadvantages, the particle filter has benefited a wide range of vision applications. Typical examples includes non-rigid object tracking \cite{nummiaro2002color, okuma2004boosted, zhang2017multi, yang2005fast, smith2005using}, simultaneous localization and mapping (SLAM) \cite{fox1999monte, karkus2018particle} and reinforcement learning (maze wondering) \cite{jonschkowski2018differentiable}. 
%Besides the similar tasks that are shared with Kalman filter, particle filter comes with more handy in terms of dealing with non-rigid vision tasks.  

Recall that the Kalman methods update state variables with the residual between prior and true measurements. In other words, there has to be a direct calculating function that transforms states to measurements for prediction and this function needs to be invertible for updates (\ie meansurement matrix, $H$, and its inverse, $H^{T}$, must exist). Notably, however, strong image features are often abstract and beyond coarse physical system measurements, \eg color histograms and motion cues can not be attained through direct projection from image coordinates and yet they can be crucial for recognizing objects under non-stationary conditions like change of view and illumination.
 \begin{figure}[ht]
    \centering
    \begin{minipage}{.15\textwidth}
    \centering
    \includegraphics[width=1.\textwidth]{Figures/pf_face.png}
    \subcaption{(a)}
    \end{minipage}
    \begin{minipage}{.25\textwidth}
    \centering
    \includegraphics[width=1.\textwidth]{Figures/face_bin_pf.png}
    \subcaption{(b)}
    \end{minipage}
    \begin{minipage}{.48\textwidth}
    \centering
    \includegraphics[width=1.\textwidth]{Figures/adaboost_pf.png}
    \subcaption{(c)}
    \end{minipage}
\caption{(a) Particle filter tracking human face with pre-collected human face color-bin as template (b) from \cite{nummiaro2002color}. (c) Multi-target tracking example in a hockey court from \cite{okuma2004boosted}.
Players, indicated by boxes, are captured by the particle filter based on color information.
Figure reproduced from \cite{nummiaro2002color} and \cite{okuma2004boosted}.}
\label{fig:face_pf_tracking}
\end{figure}
Here, the particle filter excels in working with high-level visual features. In the example of human face tracking, 
an approach has integrated color distribution features into a particle filter \cite{nummiaro2002color}; see Figure \ref{fig:face_pf_tracking} (a) and (b).
%K. Nummiaro \etal \cite{nummiaro2002color} integrate reliable color distribution features into particle filter and compare with target template using Bhattacharyya coefficient in Figure \ref{fig:face_pf_tracking}. 
Their system adopted state vectors from physical image space:
$\mathbf{x} = \{ x, y, \hat{x}, \hat{y}, L_{x}, L_{y}, \hat{L}{x}, \hat{L}_{y} \}$, where $x, y$ are image coordinates, $\hat{x}, \hat{y}$ are coordinate changes, $L_{x}, L_{y}$ are lengths of half-axes of an ellipse encompassing the target and their corresponding changes $\hat{L}_{x}, \hat{L}_{y}$. The observation, however, is the RGB color-bin distribution of the predicted ellipse window organized in 8x8x8 bin size. To update, just re-weighting each particle given the groundtruth color distribution is enough. Other such features include 3D keypoints \cite{choi2012robust}, Sobel-Edges \cite{klein2006full, choi20123d}, a combination of contour, texture and shape \cite{pistori2010mice}, and PCA based appearance features \cite{ross2008incremental}.  

The particle filter is also compatible with machine learning techniques \cite{okuma2004boosted, hess2009discriminatively} and recently has been restructured within deep neural networks. Similar to Deep-Kalman counterparts, a learnable particle filter network aims at resolving physical constraints of transition models and encouraging raw images to interact with state functions \cite{jonschkowski2018differentiable, karkus2018particle}.

\section{Gaussian Process}

A Gaussian process (GP) is a collection of random variables, any finite number of which have (consistent) Gaussian distributions. Here, by consistent, we mean for time-series data, a continuous stochastic process along the time-axis, $x_{1:t}$, can be described as a Gaussian process if and only if for every finite set of indices $1, \ldots, t$ in the index set $1, \ldots, T$, $x_{1:t}$ is a multivariate Gaussian random variable. 

A GP model is specified by its mean function, $m(x)$, and covariance function, $k(x, x^{\prime})$, which generate distributions over function $f$ as follows. Let
\begin{equation}
    m(x)  = \mathbb{E}[f(x)],
\end{equation}
\begin{equation}
    k(x, x^{\prime}) = \mathbb{E}[(f(x) - m(x)) (f(x^{\prime}) - m(x^{\prime}))],
\end{equation}
and
\begin{equation}
    f \sim \mathcal{GP}(m(x), k(x, x^{\prime})),
\end{equation}
with $\sim$ indicating generation of distributions over $f$. In the above, $x^\prime$ is used to indicate a different different point from $x$.

Notably, the mean function, $m(x)$, specifies the central value for each index $x_{t}$ whereas the variance indicates the uncertainty. To obtain a smooth trend among adjacent data points, each data point builds up co-occurance relations with all the others using the covariance function $k$. Due to this regularized inner smoothness attribute, the GP model can demonstrate very good \textbf{interpolation} results for unseen data. (An example for video data is shown in Figure \ref{fig:gauss_3dtrack}). Assuming a sequence comprises $n$ elements, its covariance matrix is then an $n \times n$ matrix.

The choice of the covariance function determines how adjacent points follow each other such that the transition can be coherent and smooth (as distinct from some zig-zag tracking results from the Kalman filter). Therefore, potential functions should assign a relatively high $k(x, x^{\prime})$ value for neighboring data.
Popular candidates are constant $k(x, x^{\prime})= C$, linear $k(x, x^{\prime})= x^{T}x$ and Radius Basis Function (RBF) $k(x, x^{\prime})= exp(-\frac{||x - x^{\prime}||^2}{2l^2})$, with $l$ related to the kernel width. Detailed comparison of various covariance functions can be found elsewhere \cite{duvenaud2014automatic}.

A common way to begin a GP model is specifying a prior mean function and a covariance function $k(x, x^{\prime})$ by experience. Most research selects a \textit{zero} mean function as prior and the covariance values are soley decided by the picked function. Sampling from such an initial choice yields unregularized results. 
%In the exmaple of choosing RBF kernel as covariance function in Figure \ref{eq:gp_fit}(a), sampled functions under the "Prior" title demonstrate a large uncertainty as well as roughly zero mean property.

Typically, one is interested in the posterior probability, $p(x|y)$, with $x$ the underlying variable of interest and $y$ the observable. Correspondingly, to instantiate a GP model it must be fit to observed data.
%However, what researchers are interested is the posterior probability $p(x|y)$, with $x$ as the researched random variable and $y$ as the observed target value. 
\iffalse
Assuming the target value $y$ is governed by $x$ and the weight matrix $w$ specified by a prior as
\fi
\iffalse
\begin{equation}
    \begin{aligned}
    y = x^{T} w + \epsilon    \\
    w \sim N(0, \Sigma_{p})
    \end{aligned}
\end{equation}
where $\epsilon$ is the noise.
\fi
\iffalse
\begin{equation}
    p(w | y, x) = \frac{p(y|x, w)p(w)}{p(y|x)}
\end{equation}
\fi
%$One necessary step prior to using Gaussian process is fitting it with real observation data $Y = \{ y_{1}, ..., y_{t} \}$ since the prior distribution for both mean and covariance functions are too coarse to model anything well. Due to the assumption of isotropic Gaussian on each $x$, one can deduct the marginalized distribution $p(X|Y)$ easily in closed form as following:
%So to instantiate a Gaussian process model, it must be fitted with observed data, $\mathbf{y}={y_1\ldots, y_t}$, from the training set. 
Due to the assumption of an isotropic Gaussiann on each $x$, one can deduce the posterior from the distribution marginalization of the joint probability of two Gaussian random variables $p(x, y)$ as
% ref: https://online.stat.psu.edu/stat505/lesson/6/6.1#:~:text=Conditional%20Distribution%20Properties&text=For%20instance%2C%20gives%20the%20means,variances%20and%20covariances%20for%20vector%20.&text=Any%20distribution%20for%20a%20subset,is%20a%20multivariate%20normal%20distribution.;
% proof of conditional gaussian.pdf: http://users.stat.umn.edu/~helwig/notes/norm-Notes.pdf;
\begin{equation}
    \centering
    \begin{aligned}
    &p(x, y) = \mathcal{N} \left(
        \begin{bmatrix}
            \mu_x \\
            \mu_y
        \end{bmatrix}
        ,
        \begin{bmatrix}
            \Sigma_{x}, \Sigma_{xy} \\
            \Sigma_{yx}, \Sigma_{y} \\
        \end{bmatrix}
        \right)\\    
    \end{aligned}
\label{eq:gp_fit}
\end{equation}
and
\begin{equation}
p(x) = \int p(x, y) dy = \mathcal{N} (\mu_x, \Sigma_x)
\label{eq:gp_fit_2}
\end{equation}
so that
\begin{equation}
    p(x|y) = &\frac{p(x, y)}{p(x)} = \mathcal{N}(\mu_{x} + \Sigma_{xy}\Sigma_{y}^{-1}(y-\mu_{y}), \;\;\; \Sigma_{x} - \Sigma_{xy}\Sigma_{y}^{-1}\Sigma_{xy}^{T}),
\label{eq:gp_fit_3}
\end{equation}
where $\mu_x$ and $\mu_y$ are mean values for prior and observations, respectively, and $\Sigma$ symbolizes the various covariance matrices defined by $k(x,x^\prime)$.
%$\Sigma$ is the covariance matrix defined by the covariance function $k(x, x^{\prime})$.

The middle figure in Figure \ref{fig:gp_demo} demonstrates samples from a trained posterior. In comparison with the ``Prior", the posterior shows fixed target values at trained data points (\ie at position $(x=2, y=1)$), the function looses uncertainty, meaning at this point its variance becomes zero). 
Following a similar idea, the calculation of posterior density of any \textbf{test point} $x_{\ast}$ (also known as the \textbf{predictive posterior} on unseen points) from a pre-trained model is tractable \cite{rasmussen2003gaussian}.
\iffalse
\begin{equation}
    p(f_{\ast} | x_{\ast}, y, x) = \mathcal{N}(\mu_{\ast}, \Sigma_{\ast}) = \mathcal{N}(k_{\ast}k_{-1}\mathbf{y}, k_{\ast\ast} - k_{\ast}k_{-1}k_{T}),
\end{equation}
\begin{equation}
    p(f_{\ast} | x_{\ast}, y, x) = \mathcal{N}(\mu_{\ast}, \Sigma_{\ast}) = \mathcal{N}(k_{\ast}k^{-1}\mathbf{y}, k_{\ast\ast} - k_{\ast}k^{-1}k^{T}),
\end{equation}
where $k_{\ast} = \{k(x_{\ast},x_{1}), k(x_{\ast},x_{2}), ..., k(x_{\ast},x_{t}) \}$, $k_{\ast\ast} = k(x_{\ast}, x_{\ast})$ and $k = \{k(x, x^{\ast}) \}$
\fi

\begin{figure}[ht]
    \centering
    \includegraphics[width=.8\textwidth]{Figures/gp.png}
    \caption{Gaussian process intuition. (Left) Given an initial (prior) GP model with $x$ being a random variable and $x \sim \mathcal{N}(0, \sigma)$, multiple distinct functions can be sampled. After trained with a real value dataset, $\mathbf{y}$, the posterior of a GP model is much confined at trained data positions (middle). (Right) The fit model can be used for performing regression with uncertainty. Seeing the x-axis as temporal stamps would naturally fit time-series data.} 
    \label{fig:gp_demo}
\end{figure} 

The application of the GP to video understanding tasks can be categorized into two main classes: \textbf{1.} static temporal process modelling and \textbf{2.} dynamic state-space modelling. 
%The first one coincides with the origin intention of inventing GP which is serving accurate non-linear regression. It focuses on fitting video data representation into GP model by reckoning the feature at each time-stamp $f_{t}$ as GP random variable. The fitted model is useful in terms of video sequence matching, anomaly detection and classification \cite{cheng2015video, kim2011gaussian, altun2004gaussian, li2015anomaly,cheng2015gaussian}.
The first coincides with the originally intended application of GPs, serving accurate nonlinear regression \cite{rasmussen2003gaussian}. In application to video, the focus is on using the model to represent a visual feature value, $f_t$, at each time, $t$, according to a GP model. Example video applications include video sequence matching, anomaly detection and classification \cite{cheng2015video, kim2011gaussian, altun2004gaussian, li2015anomaly,cheng2015gaussian}.

Another line of research incorporates GPs with state space dynamic models. As mentioned above, a vanilla Gaussian process links neighboring data points using a distance based covariance matrix (\eg an RBF kernel), which does not emphasizes any \textit{causal} relations among data points but accents on the aggregated group effect. In contrast, the Bayesian recursive filter advocates state transition functions to support information propagation to be made about future data. A dynamic function matters particularly for extrapolation tasks, which otherwise would only degrade to the prior mean value of the GP model.

To harvest the advantages of state space domain knowledge, the combination of GPs with Markov dynamic systems has been explored extensively, \eg \cite{ko2009gp, girard2003gaussian, ellis2009modelling, wang2006gaussian, urtasun20063d, wang2007gaussian, lee2016predicting, damianou2011variational}. The core of the compound is assisting GP models with latent state dynamics. 
%Once again, the state transition and observation measurement functions need to be specified. 
In this literature, a research direction formulated the desired dynamical function with GP regressions and the overall framework is referred to as Gaussian process dynamic models (GPDM) \cite{wang2006gaussian, urtasun20063d}.
As a specific example, a linear transition model, $m(x) = wx + b$, was used with a GP model to predict player reactions from American football clips \cite{lee2016predicting}. Input to the system was a sequence of trajectory features extracted from video of players and the GP model was used to regress activity labels, with the values for the parameters, $w$ and $b$, estimated via gradient descent. Other work has incorporated more complicated dynamic models (\eg another GP model that comprises linear and RBF kernels \cite{urtasun20063d}) with application to a wide variety of tasks, including human motion interpolation \cite{wang2006gaussian}, 3D people tracking \cite{urtasun20063d} and pedestrian trajectory prediction \cite{ellis2009modelling}. The latent variable is often initialized as the output from PCA dimension reduction on visual features (\eg body keypoints in \cite{urtasun20063d}) and parameters are learned via a maximum a posteriori solution.
An example applying GPDM to human tracking is shown in Figure \ref{fig:gauss_3dtrack}.

%In response, Lee \etal \cite{lee2016predicting} adopted linear transition model ($m(x) = wx + b$) for their GP model to predict the players' reactions from American football clips. They inputs a sequence of features extracted from target players and model its regression to desired labels with GP. The parameters $\{w, b\}$ is estimated with gradient descent optimization. Other work coins a set of latent states with probabilistic PCA \cite{tipping1999probabilistic, lawrence2004gaussian} from training observations and formulate their dynamic with a separate GP model. The specific dynamic of latent states is characterized through its covariance matrix. An example of such model from \cite{urtasun20063d} is as: $k(x, x^{\prime}) = exp(-\frac{|| x - x^{\prime} ||^{2}}{2l^{2}}) + x^{T}x^{\prime}$, namely a combination of Linear and RBF kernel (For extrapolations beyond training index range (0, t), $x_{t+1}$ will be decided only from early elements using this kernel combination). This technique is  phrased as Gaussian process dynamic model (GPDM), based on which some respectable applications have been built, such as human motion interpolation \cite{wang2007gaussian}, 3D people tracking \cite{urtasun20063d} and long-term pedestrian trajectory prediction \cite{ellis2009modelling}.

One unignorable disadvantage of the GP model is that it can not scale up to large sample size with ease. Since each data point will be modeled as a Gaussian, a series of spatiotemporal features with feature dimension in $\mathbb{R}^d$ and temporal scope $k$ would result in $k \times d$ multivariate Gaussians. Its covariance matrix thus ends up with $k \times k \times d$ elements, which is prohibitive under current parameter estimation literature for large $k$ and $d$.

Moreover, to estimate any involved parameter, \ie the length scale parameter of the RBF kernel for $k(x, x^{\prime})$ or the general fitting process, the space and time complexity is $\mathcal{O}(N^{3})$ (with $N$ the dataset size). Recently, some research has sought remedies for these limitations via machine learning \cite{damianou2013deep, lu2020interpretable, liu2020gaussian}; however, the applications were not to visual tasks.
%researcher seek a remedy in machine learning and deep learning \cite{damianou2013deep, lu2020interpretable,liu2020gaussian} but none has a focus on video visions. 
\begin{figure}[ht]
    \centering
    \includegraphics[width=1.\textwidth]{Figures/gp_3dtrack.png}
    \caption{3D human tracking from GPDM \cite{urtasun20063d} that interpolates the occluded frame. During interpolation, the body part exhibits natural and non-rigid movement trajectory. Figure reproduced from \cite{urtasun20063d}.}
    \label{fig:gauss_3dtrack}
\end{figure}

\section{Auto Regressive Model}
The idea of an Auto-Regressive (AR) model is to capture the auto-correlation of sequential data in a regression type model and use it to improve short-term forecasts. Its key concept is the \textbf{order} of the AR model. 
The auto-regressive model can be formally expressed as
\begin{equation}
    y_{t} = \beta_{0} + \beta_{1}y_{t-1} + \beta_{1}y_{t-2}, ..., + \beta_{t}y_{t-n} + \epsilon_{t},
\label{eq:AR}
\end{equation}
where $\beta_{t}$ is the $n_{th}$ coefficient for the corresponding delay tap version of the series data, $y_{t-n}$, and $\epsilon_{t}$ is the noise signal at the current time-step. One important assumption under the AR model is the \textbf{stationary} property, whereby statistical properties such as mean, variance, auto-correlation, etc., are all constant over time.

In the above formula, lagged data points ranging from $(t-1, t-n)$ are used to infer the data value at point $t$ and therefore it is defined as an AR model of order $n$, or an $AR(n)$ model. The order term corresponds to the same concept from higher-order Markov chains. AR is a sub-class of regression models and can be estimated through various methods such as least-squares, Maximum Likelihood \cite{doretto2003editable}, Yule-Walker equation \cite{doretto2003dynamic} or Maximum Entropy Spectral Analysis (MESA) \cite{burg1974maximum}.

In the field of video sequence analysis, \textbf{dynamic texture} \cite{doretto2003dynamic} data has been argued to have the required stationary property. Running water, flying flags or flickering flame can be viewed as stationary data in the spatiotemporal domain in the sense that they exhibit certain periodic patterns in visual spacetime. Since such patterns are pervasive in real-world videos, models of dynamic texture have been widely investigated for purposes of both analysis and synthesis. Considerable work in this area has relied on AR analytic tools \cite{cliff1975space, doretto2003dynamic,wang2002generative, hyndman2007higher, doretto2003editable, murdock2015building}. Though they differ slightly in processing of the raw image (\eg working on input pixel values \cite{cliff1975space}, PCA features \cite{hyndman2007higher}, Gabor/Laplacian decompositions \cite{wang2002generative}), all have adopted AR of various orders to model state dynamics. Figure \ref{fig:ar_dt} provides an illustrative example.
Of course, the stationary limitation makes the synthesis of video sequences that are parting from dynamic textures sub-optimal. 
Even for dynamic textures, it appears that such models tend to emphasize spatial appearance at the expense of temporal dynamics \cite{woolfe2006shift}.
Likely for these reasons, AR models are less popular than others for video prediction and synthesis.
%In the task of common video prediction or generation, AR appears much less frequently than others (See Section 3.1).  

%A. Cliff \etal \cite{cliff1975space} work on pixels, M. Hyndman \etal \cite{hyndman2007higher} work on low-dimensional PCA features and Y. Wang \etal \cite{wang2002generative} on Gabor/Laplacian decompositions), all have adopted AR for state dynamics, either in lower or higher order.
%Modelling the progression of these dynamic texture attracts attentions and AR has been found applicable for synthesizing texture movements.
\begin{figure}[ht]
    \centering
    \includegraphics[width=.8\textwidth]{Figures/ar_dt.png}
\caption{Dynamic texture example of flicking fire synthesized using higher-order AR model \cite{hyndman2007higher}. To grab a robust as well as sparse representation of frame sequences, an appearance vector of frames is obtained through principle component analysis. 
The feature dynamics are modelled as an AR process.
Figure reproduced from \cite{hyndman2007higher}.}
\label{fig:ar_dt}
\end{figure} 

\section{Recurrent Neural Networks}
In this section, we describe a type of neural network that was invented for processing sequential data, Recurrent Neural Networks (RNNs) \cite{bengio1994learning}. Artificial neurons (\eg perceptrons) are designed with inspiration from biological neurons \cite{hasson2020direct}. In essence, they follow linear combination of their inputs with various nonlinearities (\eg rectifiers, sigmoids and normalizations). Neural networks consisting of multiple layers of such neurons are devised to solve a wide variety of complicated tasks, especially those commonly associated with human intelligence. Regular NNs are feed-forward, namely a collection of directed neurons transforming the input to output without looking back, \ie they can be thought of as directed acyclic computational graphs.

In contrast, RNNs borrow power from recurrently updated hidden states to better capture inner dynamics of sequential data. Their mathematical formulation can be given as:
\begin{equation}
    h_{t} = \sigma ( {W}_{x} x_{t} +  {W}_{h} h_{t-1} + b_{h}),
\label{eq:rnn_1}
\end{equation}
so that
\begin{equation}
    y_{t} = \sigma ({W}_{y} h_{t} + b_{y}),
\label{eq:rnn_2}
\end{equation}
where ${W}_{x}, {W}_{y}, {W}_{h}$ are mapping matrices for the input, $x_{t}$, 
%output $y_{t}$ and hidden state $h_{t}$. $\sigma$ is nonlinear activation function, \ie Sigmoid, Tanh or ReLU, which allows more complicated transition for output and hidden states.
$y_t$ is the output, $h_t$ is the hidden state, $b_y$ and $b_h$ are additive biases and $\sigma$ is a nonlinear activation function (e.g., sigmoid, Tanh or ReLU) allowing for complicated transitions between output and hidden states. Figure \ref{fig:fn_rnn} provides an illustration and comparison to purely feed-forward networks.

\begin{figure}[ht]
    \centering
    \begin{minipage}{.45\textwidth}
    \centering
    \includegraphics[width=1.\textwidth]{Figures/fn_rnn.png}
    \subcaption{(a)}
    \end{minipage}
    \hfill
    \begin{minipage}{.5\textwidth}
    \centering
    \includegraphics[width=1.\textwidth]{Figures/rnn.pdf}
    \subcaption{(b)}
    \end{minipage}
\caption{(a) Depiction of the difference between feed-forward and recurrent neural networks; (b) Unrolled computational procedure of RNNs.}
\label{fig:fn_rnn}
\end{figure}

Given a sequence of input data $x_{1:T}$, the hidden state $h_{t}$ is consistently refreshed with new incoming input and the inference for output depends on the up-till-now hidden state. This particular module is referred to as a \textbf{memory} unit since it stores historical information in hidden states. In comparison, Bayesian filters and HMMs also belong to memory type models, whereas auto-regressive models and Markov Chain models are categorized as \textbf{memoryless}, since their inference relies on limited past input without updating states.

Furthermore, RNNs differ from Bayesian filters and HMMs in that their states are deterministic rather than stochastic. Some would argue that the deterministic property relaxes the trouble of inferring the hidden state and is more efficient \cite{hochreiter1997long}. The cost is that we would never know the exact state. From the perspective of recursive inference, the RNN is akin much more to the Bayesian filter in allowing for variable input and output length.

With the back-propagation algorithm being a powerful optimization tool for feed-forward NNs \cite{goodfellow2016deep}, RNNs rely on its temporal version, Back-Propagation Through Time (BPTT) to estimate the parameters. However, training RNNs is not always simple. Since the transition matrices ${W}_{x}, {W}_{y}$ and ${W}_{h}$ are shared among all time stamps, RNNs would multiply the same matrices $N$ times ($N$ is the data length) so that the output $y_{t} \propto {W}_{h}^{(N)}$, meaning that the output is proportional to the power $N$ of matrix ${W}_{h}$. During back-propagation, \textbf{gradient vanishing} or \textbf{gradient explosion} thereby happens for small values or large values in the matrix, ${W}_{h}$, respectively.

To counter the difficulity in the training, the Long-Short Term Memory \cite{hochreiter1997long} (LSTM) unit is introduced. The LSTM architecture consists of a set of recurrently connected subnets, known as memory blocks. These blocks can be thought of as a differentiable version of the memory chips in a digital computer. Each block contains one or more self-connected memory cells and three multiplicative units (forget gate $\mathbf{f}_{t}$, output gate $\mathbf{o}_{t}$ and input gate $\mathbf{i}_{t}$) that provide continuous analogues of reset, write and read operations for the cells $\mathbf{c}_{t}$ and output state $\mathbf{h}_{t}$. Figure \ref{fig:lstm} provides an architectural diagram and supporting formulae.
Note that the LSTM equations here match the vanilla RNN equations (\eg Eq. \ref{eq:rnn_1} and \ref{eq:rnn_2}) since
\begin{equation}
\begin{aligned}
     h_t &= o_{t} \circ \sigma_h (c_{t}) \\
         &= f_{t} \circ c_{t-1} + \sigma_g ({W}_{i} x_{t} + {U}_{i} h_{t-1} + b_{i}) \circ \sigma_c ({W}_{c} x_{t} + {U}_{c} h_{t-1} + b_{c}),
\end{aligned}
\end{equation}
which represents a compound mapping function: $(x_t, h_{t-1}) \rightarrow h_t$. Moreover, the mapping from hidden states to desired outputs, $h_t \rightarrow y_t$ in RNN equation \ref{eq:rnn_2}, is often neglected in the LSTM.
\begin{figure}
\begin{minipage}{.5\textwidth}
    \centering
    \includegraphics[width=.85\textwidth]{Figures/lstm.jpg}
\end{minipage}
\begin{minipage}{.45\textwidth}
\begin{flushright}
\begin{math}
\begin{aligned}
  f_{t} &= \sigma_g ({W}_{f} x_{t} + {U}_{f} h_{t-1} + b_{f}) \\
  i_{t} &= \sigma_g ({W}_{i} x_{t} + {U}_{i} h_{t-1} + b_{i}) \\
  o_{t} &= \sigma_g ({W}_{o} x_{t} + {U}_{o} h_{t-1} + b_{o}) \\
  \Tilde{c}_{t} &= \sigma_c ({W}_{c} x_{t} + {U}_{c} h_{t-1} + b_{c}) \\
  c_{t} &= f_{t} \circ c_{t-1} + i_{t} \circ \Tilde{c}_{t} \\
  h_{t} &= o_{t} \circ \sigma_h (c_{t})
\end{aligned}
\end{math}
\end{flushright}
\end{minipage}
\caption{Diagram of Long-Short Term Memory unit and its operating equations. Figure reproduced from \cite{45500}.}
\label{fig:lstm}
\end{figure}
%y_{t} &= \sigma ({W_y} h_{t} + b_y)

At every time step in LSTM processing, memory cell, $\mathbf{c}_{t}$, is decided by: \textbf{1.} the Hadamard product, $\circ$, between forget gate, $\mathbf{o}_{t}$, and previous cell memory, $\mathbf{c}_{t-1}$; \textbf{2.} the same product between the input gate, $i_{t}$, and cell activation vector, $\Tilde{\mathbf{c}}_{t}$. The reason why LSTMs can mitigate gradient problems is that the switching induced by the activation of gating functions turns the multiplicative chain into an addition chain. For example, when the input gate is closed for most elements, the update memory, $\mathbf{c}_{t}$, would be largely dependent on the previous cell state; on the other hand, when the input gate is mostly open, $\mathbf{c}_{t}$ would be the addition of previous cell values and the incoming input. In both cases, the matrix multiplication is largely avoided. A Gated Recurrent Unit network (GRU) \cite{cho2014learning} shares a similar intuition, but merges the memory cell with the state vector.

%\textbf{Application:} Present days, video vision research have been greatly relying on RNN and its variants. For unsupersively learning a strong video representation, N. Srivastava \etal \cite{srivastava2015unsupervised} adopted LSTM on sports videos (UCF-101 \cite{soomro2012ucf101}) to extrapolate unseen feature sequences and use the predictive representation to obtain comparable results. X. Shi \etal \cite{xingjian2015convolutional} incorporate convolutional layers with LSTM that allows patch-wise memory information propagation. Pedestrian trajectory predictions mainly utilizes RNNs to extrapolate potential future 2D coordinate from partial observations \cite{alahi2016social, gupta2018social}. Semantic activity anticipation \cite{abu2018will, ke2019time, zhaodiverse}. Video caption generation \cite{pei2019memory}. 

Recent research in video understanding has relied greatly on RNNs and its variants. As examples: An LSTM has been applied to sports videos (UCF-101 \cite{soomro2012ucf101}) to extrapolate unseen feature sequences \cite{srivastava2015unsupervised}; LSTMs have been agumented with convolutional layers for patch-wise memory information propagation \cite{xingjian2015convolutional}; RNNs have been used for pedestrian trajectory predictions as extrapolations from partial observations \cite{alahi2016social, gupta2018social}. Additional work leveraging RNNs for video understanding includes applications to semantic activity anticipation \cite{abu2018will, ke2019time, zhaodiverse} and caption generation \cite{pei2019memory}. Thus, applications of RNNs to video understanding have spanned relatively early vision numerical extrapolation tasks to high level semantic tasks.

\section{Summary}
All of the techniques overviewed in this chapter have seen some degree of use in video predictive understanding. Following trends elsewhere in computer vision, recent work has especially made use of neural network based approaches, with a particular emphasis on RNNs, as well as combined more classical techniques with such networks. In the next chapter, we shall see how these techniques have been applied to early action recognition and future action prediction.

==> BODY/chapter6.tex <==
\section{Conclusion}

In conclusion, as Brad Pitt and his chio wife said in \cite{BibtexKey}, NTU researchers have no life. So, go get a life!

\section{Future Work}

A few suggestions are provided for related future works:

\begin{enumerate}

\item Bla.. 

\item Bla..

\item Bla..

\end{enumerate}
